Estimating Quantum Gravity Corrections to Correlators near Black Holes

We analyze the size of quantum gravity effects near black hole horizons. By considering black holes in asymptotically AdS spacetime, we can make use of the "quantum deviation" to estimate the size of quantum gravity corrections to the semiclassical analysis. We find that, in a typical pure state, corrections to correlation functions are typically of order exp(-S/2). Both the magnitude and time dependence of the correlator differ from previous results related to the spectral form factor, which estimated the correlator in a thermal state. Our results severely constrain proposals, such as non-violent unitarization and some versions of fuzzballs, that predict significant corrections to the semiclassical computation of correlation functions near black holes. We point out one possible loophole: our results rely on the standard result that bulk reconstruction is state independent for small perturbations outside the black hole.

==> introetc.tex <==
Abstract:
We analyze the size of quantum gravity effects near black hole horizons. By considering black holes in asymptotically AdS spacetime, we can make use of the quantum deviation to estimate the size of quantum gravity corrections to the semiclassical analysis. We find that, in a typical pure state, corrections to correlation functions are typically of order exp(-S/2). Both the magnitude and time dependence of the correlator differs from the spectral form factor, which captures the correlator in a thermal state. Our results severely constrain proposals, such as non-violent unitarization and some versions of fuzzballs, that predict significant corrections to the semiclassical computation of correlation functions near black holes.

Introduction:
The black hole information problem demonstrated that quantum gravity effects can become important at distance scales much longer than the Planck scale in the vicinity of black holes, raising the possibility that they may be observable. Recently, significant progress has been made in computing the quantum gravity corrections prevent information loss. Although quantum gravity effects are large in the computation of the entropy of the Hawking radiation, the entropy is not an observable quantity. 

It is an open question whether quantum gravity effects are significant for observable quantities, such as correlation functions of gravitons and other light fields. In some models, such as non-violent unitarization \cite{Giddings:2012gc, Giddings:2016plq, Giddings:2017jts} and versions of the fuzzball proposal, quantum corrections to correlators are significant near the horizon. Concretely, in the simplest version of non-violent unitarization, the two-point function of the gravitational field differs at order one from the semiclassical computation at distance and time scales of order the Schwarzschild radius. In non-violent unitarization, the two-point function of the metric perturbation in a typical pure state depends strongly on the state; this is essential for information to get out of the black hole in this model.

On the other hand, it is widely believed that corrections to correlation functions are exponentially small in the black hole entropy. Corrections of this order are sufficient to restore unitarity. In this paper we will compute the size of these corrections for black holes in asymptotically AdS spacetime.
The central question we seek to address is whether the microstates of a black hole can be probed or inferred by examining quantum operators localized near the event horizon. Specifically, we ask: to what extent is an operator $O$ outside the event horizon sensitive to these quantum microstates? 

To calculate this, we use the notion of `quantum deviation' of an operator $O$, defined by \cite{Freivogel:2021ivu}
\begin{equation}
\Delta_O^2=\int d \psi f(\psi)\left(|\langle\psi|O| \psi\rangle|^2\right)-\left(\int d \psi f(\psi)|\langle\psi|O| \psi\rangle|\right)^2,
\end{equation}
where $f(\psi)$ denotes a probability distribution over an ensemble of states. This $\Delta_O$ is designed to capture the average fluctuations, in an ensemble of states, in the {\it expectation value} of the operator $O$. It differs from the more standard quantity $\bra{\psi}O^2\ket{\psi}$; our quantity captures to what extent $\bra{\psi}O\ket{\psi}$ varies over some ensemble of states $\ket{\psi}$. As a result, this quantity is perfectly suited to asking to what extent operators outside the black hole are sensitive to the black hole microstate. 

\subsection{Summary of Results}
\paragraph{Magnitude.}
We find that quantum corrections are of order
\begin{equation}
\Delta_O^2 \sim e^{- S}
\end{equation}
where $S$ is the Bekenstein-Hawking entropy of the black hole. This corresponds to a typical difference in correlators of
\begin{equation}
\bra{\psi} O \ket{\psi} - \overline{\bra{\psi} O \ket{\psi}} \sim e^{-S/2}
\end{equation}
where the barred quantity is the ensemble average.
Considering the special case where $O$ is a long-time correlator, $O = A(t) A(0)$, our result gives
\begin{equation}
\bra{\psi} A(t) A(0) \ket{\psi} \sim e^{-S/2}
\end{equation}
This should be contrasted with computations related to the spectral form factor, which give
\begin{equation}
    \expval{A(t) A(0)}_\beta \sim e^{-S}
\end{equation}
This is not in conflict: the correlator in a typical pure state is much larger than the thermal correlator, albeit still exponentially small.
\paragraph{Time Dependence.}
...
\paragraph{Regime of Validity.}
We demonstrate that the key formula, which relates the quantum deviation to a two-sided correlator in the thermofield double state, is reliable for any operator as long as the entropy is large.

Our black hole computation is special in various ways- we focus on particular dimensions and particular modes of the gravitational fluctuations. We expect that our results will go through more generally, but have not shown this rigorously.

\subsection{Discussion}
We discuss some possible loopholes in our constraints. In particular, our results rely on the state-independent reconstruction of operators outside the horizon in the context of AdS/CFT. This type of reconstruction is standard for physics outside the horizon. One way to escape our conclusions is to claim that the same quantum corrections posited in non-violent unitarization result in state-dependent modifications of the bulk-boundary dictionary. 
%In this research, we apply the concept of quantum deviation to quantify the fluctuations of black hole metrics. We initiate our analysis by perturbing the black hole metric and proceed to study its Fourier modes. These modes are treated as bulk operators that can be mapped to the boundary via holographic bulk reconstruction techniques. Applying the concept of quantum deviation, we then compute the fluctuations of the associated boundary operators. Our preliminary findings indicate that for a 5-dimensional AdS planar black hole, fluctuations in the scalar channel of metric perturbations do not reach the $O(1)$ level. This result may offer initial guidance for testing various theoretical proposals about this topic. 

%The thesis is organized in a manner to guide the reader through each developmental phase of the research. Section 2 will offer a brief review of the quantum deviation concept and its mathematical properties. In section 3 will introduce the reader to the notion of black hole perturbation modes, and outline some details through specific calculations. Section 4 will focus on holographic bulk reconstruction, particularly emphasizing the HKLL mechanism \cite{Hamilton:2006az, Hamilton:2005ju, Leichenauer:2013kaa}, and how the perturbation modes of the black hole can be mapped onto boundary operators. Section 5 will involve calculations of boundary operator fluctuations using the quantum deviation formula, followed by an discussion on the results and their implications. Section 6 will serve as the conclusion, summarizing the research and outlining potential future directions.

For the calculations in this thesis, we employ the $(-,+,+,+)$ metric signature convention and work in Planck units $\hbar=c=G=k_B=1$. 


